Sem-DPO: Mitigating Semantic Inconsistency in Preference Optimization for Prompt Engineering

Generative AI can now synthesize strikingly realistic images from text, yet output quality remains highly sensitive to how prompts are phrased. Direct Preference Optimization (DPO) offers a lightweight, off-policy alternative to RL for automatic prompt engineering, but its token-level regularization leaves semantic inconsistency unchecked as prompts that win higher preference scores can still drift away from the user's intended meaning. We introduce Sem-DPO, a variant of DPO that preserves semantic consistency yet retains its simplicity and efficiency. Sem-DPO adjusts the DPO loss using a weight based on how different the winning prompt is from the original, reducing the impact of training examples that are semantically misaligned. We provide the first analytical bound on semantic drift for preference-tuned prompt generators, showing that Sem-DPO keeps learned prompts within a provably bounded neighborhood of the original text. On three standard text-to-image prompt-optimization benchmarks and two language models, Sem-DPO achieves 8-12% higher CLIP similarity and 5-9% higher human-preference scores (HPSv2.1, PickScore) than DPO, while also outperforming state-of-the-art baselines. These findings suggest that strong flat baselines augmented with semantic weighting should become the new standard for prompt-optimization studies and lay the groundwork for broader, semantics-aware preference optimization in language models.

==> sections/Bigtable.tex <==
% \begin{table*}[htbp]
% \centering
% \label{res}
% \small
% \scalebox{1.}{
% \begin{tabular}{p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
% \toprule
% \multicolumn{2}{c}{Human Input} & \multicolumn{2}{c}{{Promptist \citep{hao2022optimizing}}} & \multicolumn{2}{c}{{\textsc{DPO-Promptist} \textbf{(Ours)}}} \\
% \midrule
% % \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{Puppy drinking tea in space,}} & \multicolumn{2}{c}{{High resolution photo of puppy}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{painting by gaston bussiere,}} & \multicolumn{2}{c}{{drinking tea in space, trending}} \\
% \multicolumn{2}{c}{{Puppy drinking tea in space.}} & \multicolumn{2}{c}{{craig mullins, greg}} & \multicolumn{2}{c}{{on Artstation, pixiv,}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{rutkowski, alphonse mucha}} & \multicolumn{2}{c}{{hyperdetailed. RPG Portrait. 8K}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{outstanding artistic}} & \multicolumn{2}{c}{{Resolution, HD, Detailed}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{style.}} & \multicolumn{2}{c}{{Dramatic Lighting by Brom.}} \\

% \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}

% \raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/111.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/112.jpeg}} & \raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/121.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/122.jpeg}} & \raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/131.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/132.jpeg}} \\

% \midrule

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{Cute sheeps playing football}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{Cute sheeps playing football. }} & \multicolumn{2}{c}{{in the garden of Eden. high quality,}} \\
% \multicolumn{2}{c}{{Cute sheeps playing football.}} & \multicolumn{2}{c}{{3D render excited 3D visual}} & \multicolumn{2}{c}{{2D render, award winning art,}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{painting by Greg Rutkowski}} & \multicolumn{2}{c}{{photorealistic, vaporwave lighting,}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{and Tim Rutkowski and Alena.}} & \multicolumn{2}{c}{{natural, digital Art, by Makoto}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{Shinkai and Simon Stålenhag.}} \\

% \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}

% \raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/211.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/212.jpeg}} & \raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/221.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/222.jpeg}} & \raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/231.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/232.jpeg}} \\

% \midrule

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{A wooden house next to a lake }} & \multicolumn{2}{c}{{The house is next to a lake and a}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{and a lush green garden with}} & \multicolumn{2}{c}{{big colourful garden with a green}} \\
% \multicolumn{2}{c}{{A wooden house next to a}} & \multicolumn{2}{c}{{colorful flowers. Wooden}} & \multicolumn{2}{c}{{oak. Natural light, fantasy,}} \\
% \multicolumn{2}{c}{{lake and a lush green }} & \multicolumn{2}{c}{{furniture, multi-colored,}} & \multicolumn{2}{c}{{greenland, miniature, detailed}} \\
% \multicolumn{2}{c}{{garden with colorful flowers.}} & \multicolumn{2}{c}{{welcoming, 8k, detail, sharp,}} & \multicolumn{2}{c}{{concept art, epic fantasy, clouds,}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{intricate, artstation, cinematic.}} & \multicolumn{2}{c}{{realistic render, 8k, sunlight.}} \\

% \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}

% \raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/311.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/312.jpeg}} & \raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/321.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/322.jpeg}} & \raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/331.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.3cm,height=2.3cm]{sections/Template-2024/images/finImages/332.jpeg}} \\

% \bottomrule
% \end{tabular}
% }
% \caption{Images generated using human input, Promptist \citep{hao2022optimizing}, and \textsc{DPO-Promptist} prompts with Stable Diffusion v1.5 are presented in groups, each consisting of two images produced with distinct random seeds. \textsc{DPO-Promptist} images tend to yield better images compared to the original user input.}
% \label{tab:human_input_vs_promptist_vsDPO_promptist}
% \end{table*}


% ###########################

% \begin{table*}[h]
% \centering
% \label{res}
% \small
% \scalebox{.9}{
% \begin{tabular}{p{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}}
% \toprule
% \multicolumn{2}{c}{Human Input} & \multicolumn{2}{c}{{BeautifulPrompt \citep{cao2023beautifulprompt}}} & \multicolumn{2}{c}{{Promptist \citep{hao2022optimizing}}} & \multicolumn{2}{c}{{\textsc{DPO-Promptist} \textbf{(Ours)}}} \\
% \midrule

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{masterpiece, best quality, high res,}} & \multicolumn{2}{c}{{Puppy drinking tea in space,}} & \multicolumn{2}{c}{{High resolution photo of puppy}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{perfect, absurdres, drinking tea}} & \multicolumn{2}{c}{{painting by gaston bussiere,}} & \multicolumn{2}{c}{{drinking tea in space, trending}} \\
% \multicolumn{2}{c}{{Puppy drinking tea in space.}} & \multicolumn{2}{c}{{from space, looking at viewer,}} & \multicolumn{2}{c}{{craig mullins, greg}} & \multicolumn{2}{c}{{on Artstation, pixiv,}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{small dog', 'A happy puppy}} & \multicolumn{2}{c}{{rutkowski, alphonse mucha}} & \multicolumn{2}{c}{{hyperdetailed. RPG Portrait. 8K}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{drinks teapodially in space,}} & \multicolumn{2}{c}{{outstanding artistic}} & \multicolumn{2}{c}{{Resolution, HD, Detailed}} \\
% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{beautiful eyes, natural lighting,}} & \multicolumn{2}{c}{{style.}} & \multicolumn{2}{c}{{Dramatic Lighting by Brom.}} \\

% \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}

% \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/111.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/112.jpeg}} & 
% \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/141.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/142.jpeg}} & 
% \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/121.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/122.jpeg}} & \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/131.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/132.jpeg}} \\

% \midrule

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{Sheepdog, cuteness, playful, foot-}} & \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{Cute sheeps playing football}} \\

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{ball, Sheep Dogs, Sheepdog Foot-}} & \multicolumn{2}{c}{{Cute sheeps playing football. }} & \multicolumn{2}{c}{{in the garden of Eden. high quality,}} \\

% \multicolumn{2}{c}{{Cute sheeps playing football.}} &  \multicolumn{2}{c}{{ball, Furry, 4K, HQ, RAW photo,}} &
% \multicolumn{2}{c}{{3D render excited 3D visual}} & \multicolumn{2}{c}{{2D render, award winning art,}} \\

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{cute sheeps playing football, per-}} & \multicolumn{2}{c}{{painting by Greg Rutkowski}} & \multicolumn{2}{c}{{photorealistic, vaporwave lighting,}} \\

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{fect skin, matte painting, artstation,}} & \multicolumn{2}{c}{{and Tim Rutkowski and Alena.}} & \multicolumn{2}{c}{{natural, digital Art, by Makoto}} \\

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{concept art, detailed face}} & \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{Shinkai and Simon Stålenhag.}} \\

% \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}

% \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/211.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/212.jpeg}} & 
% \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/241.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/242.jpeg}} & 
% \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/221.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/222.jpeg}} & \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/231.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/232.jpeg}} \\

% \midrule

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{wooden house next to lake,}} & \multicolumn{2}{c}{{A wooden house next to a lake }} & \multicolumn{2}{c}{{The house is next to a lake and a}} \\

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{lush green garden, purple flowers,}} & \multicolumn{2}{c}{{and a lush green garden with}} & \multicolumn{2}{c}{{big colourful garden with a green}} \\

% \multicolumn{2}{c}{{A wooden house next to a}} & 
% \multicolumn{2}{c}{{yellow flowers, white flowers,}} &
% \multicolumn{2}{c}{{colorful flowers. Wooden}} & \multicolumn{2}{c}{{oak. Natural light, fantasy,}} \\

% \multicolumn{2}{c}{{lake and a lush green }} & 
% \multicolumn{2}{c}{{large flowers, Best quality, mast-}} &
% \multicolumn{2}{c}{{furniture, multi-colored,}} & \multicolumn{2}{c}{{greenland, miniature, detailed}} \\

% \multicolumn{2}{c}{{garden with colorful flowers.}} & 
% \multicolumn{2}{c}{{erpiece, ultra high res, raw photo}} &
% \multicolumn{2}{c}{{welcoming, 8k, detail, sharp,}} & \multicolumn{2}{c}{{concept art, epic fantasy, clouds,}} \\

% \multicolumn{2}{c}{{}} & \multicolumn{2}{c}{{an abandoned wooden house}} & \multicolumn{2}{c}{{intricate, artstation, cinematic.}} & \multicolumn{2}{c}{{realistic render, 8k, sunlight.}} \\

% \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}

% \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/311.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/312.jpeg}} &
% \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/341.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/342.jpeg}} &
% \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/321.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/322.jpeg}} & \raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/331.jpeg}}&\raisebox{-0.5\height}{\includegraphics[width=2.1cm,height=2.1cm]{sections/Template-2024/images/finImages/332.jpeg}} \\

% \bottomrule
% \end{tabular}
% }
% \caption{Images generated using human input, BeautifulPrompt~\citep{cao2023beautifulprompt}, Promptist~\citep{hao2022optimizing}, and \textsc{DPO-Promptist} prompts with Stable Diffusion v1.5 are presented in groups, each consisting of two images produced with distinct random seeds. \textsc{DPO-Promptist} images tend to yield better images compared to the original user input.}
% \label{tab:human_input_vs_promptist_vsDPO_promptist}
% \end{table*}




==> sections/Methods.tex <==
\section{Methods}
\label{sec:Methods}

The goal of our prompt adaptation framework is to perform prompt optimization automatically. Given user input for a text-to-image generator, our model learns to generate human-preferred prompts that obtain better output images while preserving their original intentions. The prompt optimization model is named \textsc{DPO-Promptist}, which is built upon a pre-trained language model, such as GPT-2 \citep{radford2019language}. We first conduct supervised fine-tuning (SFT) (Section~\ref{sec:supervised}). Next, we collect human preferences to curate preference data for DPO (Section~\ref{sec:PrefData}), then we fine-tune the SFT model using DPO on the preference data (Section~\ref{sec:DPO}), which improves both relevance and quality of generated images.

\subsection{Supervised Fine-tuning}
\label{sec:supervised}
The first step of our framework involves supervised fine-tuning of a language model on a set of prompt pairs. A parallel prompt corpus $D = {(x, y)}$ contains pairs of original user inputs $x$ and manually engineered examples $y$. The training objective is to maximize the log-likelihood with teacher forcing, as shown in Equation~\ref{eq:sft}:

\begin{equation}
\mathcal{L_\text{SFT}} = -\mathbb{E}_{(x,y)\sim D} \log p(y|x)
\label{eq:sft}
\end{equation}

Where $p(y|x)$ represents the conditional probability of the target prompt $y$ given the input prompt $x$.

In our experiments, we compare our work to the approach of \citep{hao2022optimizing}, and thus we employ their provided SFT GPT-2 model. They fine-tuned the GPT-2 on human-engineered prompts from the Lexica \footnote{\url{https://lexica.art/}} dataset, incorporating a main content section describing the user's intention and modifiers that customize the art style, such as artist names and popular elements. Human-engineered prompts serve as the target outputs during fine-tuning.

\subsection{Collecting Human Preferences}
\label{sec:PrefData}
We collect human preferences to fine-tune the SFT model with the DPO. For this purpose, we randomly select 100k prompts from the 1.2M prompts used by \citep{hao2022optimizing} for training the RL policy. This subset comprises in-domain prompts from the DiffusionDB dataset \citep{wang2022diffusiondb}, out-of-domain image captions from the COCO dataset \citep{chen2015microsoft}, and image labels from ImageNet-21k \citep{deng2009imagenet}. The rationale behind reducing the original dataset from 1.2M to 100k prompts is to highlight the ability of DPO to operate with a substantially smaller dataset compared to RL methods. 
% Previous works have demonstrated that DPO requires preference data with fewer samples \citep{tian2023fine}. Additionally, this approach enhances computational efficiency.
Prior research has shown that DPO can achieve competitive results with fewer preference data samples \citep{tian2023fine}, which also offers the added benefit of improved computational efficiency.

To collect human preferences, we utilize ImageReward \citep{xu2024imagereward}, an automatic text-to-image evaluation metric. We generate two outputs for each of the 100k prompts from the SFT model. Subsequently, we employ Stable Diffusion \citep{rombach2022high} v1.4\footnote{\url{https://huggingface.co/CompVis/stable-diffusion-v1-4}} to generate one image for each of the two prompts. To accelerate the image generation process, we employed the Denoising Diffusion Implicit Models (DDIM) scheduler \citep{song2020denoising}, which leverages a more efficient sampling approach compared to the default scheduler. For each generated image, we compute an ImageReward score and use these scores to rank the images. We label the prompt with the higher score as the accepted prompt and the other as the rejected prompt, thereby creating the preference data as shown in step 2 in figure~\ref{fig:fig1}.


\subsection{Direct Preference Optimization}
\label{sec:DPO}
We employ the Direct Preference Optimization (DPO) algorithm to streamline RL on language models (LMs). This approach specifically addresses scenarios involving preference-based optimization of LMs \citep{rafailov2023direct}. The DPO method relies on a dataset of preference pairs $D = \{x^{(i)}, y_w^{(i)}, y_l^{(i)}\}_{i=1}^N$ consisting of prompts $x$ and candidate responses $y_w$ and $y_l$, where $y_w$ is preferred over $y_l$ (indicated as $y_w \succ y_l$). The selection of $y_w$ over $y_l$ depends on the application where DPO is being used. These preferences can be collected either by human annotators or models that mimic human behavior \citep{wu2023human, kirstain2024pick, xu2024imagereward}. The likelihood of observing a specific preference pair follows the Bradley-Terry model, which measures how well a given reward function aligns with preference data \citep{bradley1952rank}:

\begin{align}
p(y_w > y_l) = \sigma(r(x, y_w) - r(x, y_l)) \label{eq:2}
\end{align}

Here, $\sigma$ denotes the sigmoid function, and $r(x, y)$ signifies an unobserved reward or scoring function. As demonstrated by Rafailov et al. (2023), the optimal policy $\pi^*$ can be derived by optimizing a loss directly computed on the preference data:

\begin{align}
L_{\text{DPO}}(\pi_{\theta}; \pi_{\textrm{ref}}, D) = -\mathbb{E}_{(x, y_w, y_l) \sim D} \notag \\
\biggl\{ \log \biggl[\sigma \biggl( \beta \log \frac{\pi_{\theta}(y_w | x)}{\pi_{\textrm{ref}}(y_w | x)} - \beta \log \frac{\pi_{\theta}(y_l | x)}{\pi_{\textrm{ref}}(y_l | x)} \biggr) \biggr] \biggr\} \label{eq:1}
\end{align}

Here, DPO aims to learn a parameterized policy $\pi_{\theta}$ from a fixed dataset of preferences, with $\beta$ being a tuning parameter. The $\pi_{\textrm{ref}}$ is a reference or baseline policy used to normalize or compare the performance of the policy being optimized. Specifically, we set $\pi_{\textrm{ref}}$ to be the pre-trained language model and fine-tune $\pi_{\theta}$ on our curated dataset to surpass this reference model.

DPO enables learning of $\pi_{\theta}$ from a preferences dataset without the need for fitting an explicit reward function. In the preference dataset, we regard prompts with higher ImageReward scores as $y_w$ and prompts with lower ImageReward scores as $y_l$ in Equation \ref{eq:2}, respectively. We then run DPO for five epochs with a learning rate of 5e-5. We show the convergence of the loss function in Figure \ref{fig:loss} in Appendix \ref{sec:App}.

==> sections/SDPO.tex <==
\section{Sematic-DPO: Semantic Direct Preference Optimization}

Although DPO effectively trains the model to assign a higher probability to preferred responses compared to dispreferred ones, it does not explicitly ensure that the generated responses, particularly the preferred ones, remain semantically grounded in the original input prompt $x$. This can potentially lead to scenarios where the model learns to satisfy preferences but generates outputs that drift semantically from the user's intent or the context provided in the prompt. To address this potential for semantic drift and encourage the model to generate preferred responses that are also semantically relevant to the input, we propose Semantic Direct Preference Optimization (Semantic-DPO). Semantic-DPO modifies the standard DPO objective by introducing a weighting factor for each preference pair, where the weight is determined by the semantic similarity between the input prompt $x$ and the preferred response $y_w$ by the given equation:

{\small
\[
W(x, y_w) = \exp\biggl(-\alpha.d\Bigl(e_{\phi}(x), e_{\phi}(y_w) \Bigr) \biggr)
\]
}
where $W(x, y_w)$ is a weighting function that increases with the semantic similarity between $x$ and $y_w$. We compute this semantic similarity using a fixed, pre-trained external embedding model $e_\phi$ (e.g., a Sentence Transformer or a CLIP text encoder) to obtain stable semantic representations of $x$ and $y_w$. The weighting function is then defined based on a semantic distance metric $d(e_\phi(x), e_\phi(y_w))$, where $d(\cdot,\cdot)$ is a distance (e.g., $1-\text{cosine-similarity}$) and $\alpha \ge 0$ is a hyperparameter that controls the strength of the semantic weighting. 
A higher value of $\alpha$ assigns lower weights to preference pairs with larger semantic distance between $x$ and $y_w$, effectively reducing their influence on the DPO loss. Conversely, pairs with high semantic similarity between $x$ and $y_w$ receive weights closer to 1, retaining their full influence on the loss.

This approach prioritizes learning from preference pairs where the preferred response is already semantically aligned with the input, implicitly guiding the model towards generating relevant and preferred outputs. The WSDPO loss function for a single preference pair $(x, y_w , y_l)$ is defined as:

{\small
\[
\begin{split}
\mathcal{L}_{\text{Semantic-DPO}}(\theta) = - W(x, y_w). \\
\log \Biggl( \sigma \biggl( \beta \Bigl( 
\log \frac{\pi_\theta(y_w|x)}{\pi_{ref}(y_w|x)} - \frac{\pi_\theta(y_l|x)}{\pi_{ref}(y_l|x)} \Bigr) \biggr) \Biggr)
\end{split}
\]
}

% \textbf{Mechanism and Impact on Policy:}
% The WSDPO loss is minimized using gradient descent with respect to the parameters $\theta$ of the trainable policy $\pi_\theta$. The gradient of the WSDPO loss is given by:

% \[
% \begin{split}
% \nabla_\theta \mathcal{L} \theta 
% \Biggl[ \log \Biggl( \sigma \biggl( \beta \Bigl( 
% \log \frac{\pi_\theta(y_w|x)}{\pi_{ref}(y_w|x)} - \frac{\pi_\theta(y_l|x)}{\pi_{ref}(y_l|x)} \Bigr) \biggr) \Biggr) \Biggr]
% \end{split}
% \]

% This shows that the gradient is the standard DPO gradient, scaled by the weighting factor $W(x, y_w)$. Since $W(x, y_w)$ is pre-computed based on a fixed embedder and the dataset, it acts as a constant scaling factor for the gradient of each sample within a batch. This implicitly guides the training process by: 
% \textbf{prioritizing Relevant Samples}: Preference pairs where the preferred response $y_w$ is semantically close to the input $x$ (resulting in a high $W(x, y_w)$ will contribute more significantly to the overall gradient and thus have a larger impact on updating the model's parameters.
% \textbf{Downweighting Irrelevant Samples}: Preference pairs where $y_w$ is semantically distant from $x$ (resulting in a low $W(x, y_w)$ will have their corresponding DPO loss and gradient downweighted, reducing their influence on the training.

% This mechanism allows the model to primarily learn its preference alignment from data that is already aligned with the desired semantic relevance property, without adding a separate loss term that might introduce conflicting gradients or primarily affect only specific layers like the embedding layer. The semantic signal from the fixed embedder is used to modulate the learning signal derived from the human preferences.

% \paragraph{Theoretical Considerations and Guarantees.}
% The original DPO framework provides theoretical guarantees related to optimizing an implicit reward function and controlling divergence from the reference policy. By introducing the weighting factor $W(x,y_w)$, WSDPO effectively changes the distribution of data from which the model learns. Instead of optimizing the DPO objective over the uniform distribution of preference pairs in the dataset $D$, WSDPO optimizes it over a re-weighted distribution $D'$ where the weight of each sample $(x, y_w, y_l)$ is proportional to $W(x,y_w)$.

% While the core DPO objective form is preserved, the theoretical guarantees of standard DPO do not directly apply to this re-weighted optimization without further analysis. Future theoretical work could explore the properties of the implicit reward function and the policy convergence when optimizing the DPO loss under a data distribution weighted by semantic relevance. However, empirically, this weighting is expected to steer the model towards a policy that is not only good at satisfying preferences but also biased towards generating outputs semantically related to the input, particularly for inputs similar to those in the training data.

% \textbf{Practical Implementation and Hyperparameter Tuning:}
% Implementing WSDPO requires selecting a suitable fixed external embedding model $e_\phi$ and a semantic distance metric $d$. The weighting factor $W(x,y_w)$ can be pre-computed for the entire dataset before training or computed on-the-fly for each batch. The hyperparameter $\alpha$ controls the strength of the semantic weighting. Tuning $\alpha$ is crucial to balance the influence of the semantic signal with the original preference signal. If $\alpha$ is too high, the model might overly prioritize semantic similarity and potentially ignore preferences from pairs where $y_w$ is preferred despite some semantic distance. If $\alpha$ is too low, the semantic weighting will have little effect. We recommend using a validation dataset and evaluating performance on both preference satisfaction (e.g., win rate on validation preferences) and semantic relevance (e.g., average semantic similarity between generated outputs and prompts on a validation set, or human evaluation) to find the optimal value for $\alpha$.


==> sections/Tables/new_table.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{c|lccccccccc}
\noalign{\hrule height 1pt} 
\multirow{2}{*}{\footnotesize \textbf{\begin{tabular}[c]{@{}c@{}}Language\\ Model\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\footnotesize\textbf{Optimizations}}} & \multicolumn{6}{c|}{\footnotesize\textit{\textbf{Levels}}} & \multirow{2}{*}{\footnotesize \textbf{\begin{tabular}[c]{@{}c@{}}Total\\ Accuracy\end{tabular}}} \\ \cline{3-8} 
 & \multicolumn{1}{c|}{} & \footnotesize\textbf{1 $(\uparrow)$} & \multicolumn{1}{c}{\footnotesize\textbf{2 $(\uparrow)$}} & \footnotesize\textbf{3 $(\uparrow)$} & \multicolumn{1}{c}{\footnotesize\textbf{4 $(\uparrow)$}} & \footnotesize\textbf{5 $(\uparrow)$} & \multicolumn{1}{c|}{\footnotesize\textbf{6 $(\uparrow)$}} \\

\hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{CodeLlama 7b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 10 & 0 & 10 & 0 & 10 & \multicolumn{1}{l|}{0} &  \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 0 & 0 & 0 & 0 & 0 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 10 & 0 & 20 & 0 & 10 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 40 & 0 & 100 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{Combinations}} & \cellcolor{pink!50}40 & \cellcolor{pink!50}30 & \cellcolor{pink!50}100 & \cellcolor{pink!50}0 & \cellcolor{pink!50}30 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \\
\hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{CodeLlama 13b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 10 & 0 & 10 & 0 & 10 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 10 & 0 & 10 & 0 & 0 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 20 & 10 & 10 & 0 & 10 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 60 & 90 & 90 & 0 & 20 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{Combinations}} & \cellcolor{pink!50}90 & \cellcolor{pink!50}80 & \cellcolor{pink!50}80 & \cellcolor{pink!50}10 & \cellcolor{pink!50}30 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \\
\hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{Llama 3.1 8b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 30 & 0 & 40 & 0 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 0 & 0 & 30 & 0 & 20 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 40 & 0 & 40 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 100 & 60 & 100 & 100 & 60 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{Combinations}} & \cellcolor{pink!50}90 & \cellcolor{pink!50}30 & \cellcolor{pink!50}100 & \cellcolor{pink!50}30 & \cellcolor{pink!50}50 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \\
\hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{DeepSeekV2 16b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 10 & 0 & 10 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 20 & 30 & 30 & 0 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 10 & 10 & 20 & 0 & 20 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 80 & 80 & 100 & 0 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{Combinations}} & \cellcolor{pink!50}80 & \cellcolor{pink!50}80 & \cellcolor{pink!50}100 & \cellcolor{pink!50}0 & \cellcolor{pink!50}40 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \\
\hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{Qwen2.5 7b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 30 & 30 & 30 & 0 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 40 & 0 & 30 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 20 & 30 & 10 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 90 & 90 & 100 & 0 & 50 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{Combinations}} & \cellcolor{pink!50}100 & \cellcolor{pink!50}90 & \cellcolor{pink!50}100 & \cellcolor{pink!50}0 & \cellcolor{pink!50}50 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \\
\hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{Qwen2.5 14b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 90 & 60 & 90 & 10 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 80 & 50 & 70 & 20 & 50 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 20 & 30 & 10 & 0 & 30 & \multicolumn{1}{l|}{20} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 100 & 90 & 100 & 0 & 50 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{Combinations}} & \cellcolor{pink!50}100 & \cellcolor{pink!50}90 & \cellcolor{pink!50}100 & \cellcolor{pink!50}40 & \cellcolor{pink!50}50 & \multicolumn{1}{l|}{\cellcolor{pink!50}30} & \\
\hline
\hline

\noalign{\hrule height 1pt}
\end{tabular}
\caption{Comparison of automatic prompt optimization methods in Text-to-Image Generation across automated evaluation metrics and human preference metrics}
\label{table:main_small}
\end{table*}
